A new class of $\alpha$-Farey maps and an application to normal numbers

We define two types of the $\alpha$-Farey maps $F_{\alpha}$ and $F_{\alpha, \flat}$ for $0 < \alpha < \tfrac{1}{2}$, which were previously defined only for $\tfrac{1}{2} \le \alpha \le 1$ by R.~Natsui (2004). Then, for each $0 < \alpha < \tfrac{1}{2}$, we construct the natural extension maps on the plane and show that the natural extension of $F_{\alpha, \flat}$ is metrically isomorphic to the natural extension of the original Farey map. As an application, we show that the set of normal numbers associted with $\alpha$-continued fractions does not vary by the choice of $\alpha$, $0 < \alpha < 1$. This extends the result by C.~Kraaikamp and H.~Nakada (2000).

==> Figure1DataLeftFunction.tex <==
#Curve 0, 16 points
#x y type
-0.75 3 i
-0.7 2.3333 i
-0.65 1.857143 i
-0.6 1.5 i
-0.55 1.2222 i
-0.5 1 i
-0.45 0.8182 i
-0.4 0.6667 i
-0.35 0.53846 i
-0.3 0.42857 i
-0.25 0.33333 i
-0.2 0.25 i
-0.15 0.17647 i
-0.1 0.11111 i
-0.05 0.05263 i
0 0 i


==> Figure1DataMiddleFunction.tex <==
#Curve 0, 17 points
#x y type
0 0 i
0.05 0.0526 i
0.1 0.1111 i
0.15 0.1764706 i
0.2 0.25 i
0.25 0.33333 i
0.3 0.4285714 i
0.35 0.5384615 i
0.4 0.6666667 i
0.45 0.8181818 i
0.5 1 i
0.55 1.222222 i
0.6 1.5 i
0.65 1.857143 i
0.7 2.333333 i
0.75 3 i
0.8 4 i


==> Figure1DataRightFunction.tex <==
#Curve 0, 65 points
#x y type
0.8 0.25 i
0.85 0.1764706 i
0.9 0.1111111 i
0.95 0.05263158 i
1 0 i
1.05 -0.04761905 i
1.1 -0.09090909 i
1.15 -0.1304348 i
1.2 -0.1666667 i
1.25 -0.2 i
1.3 -0.2307692 i
1.35 -0.2592593 i
1.4 -0.2857143 i
1.45 -0.3103448 i
1.5 -0.3333333 i
1.55 -0.3548387 i
1.6 -0.375 i
1.65 -0.3939394 i
1.7 -0.4117647 i
1.75 -0.4285714 i
1.8 -0.4444444 i
1.85 -0.4594595 i
1.9 -0.4736842 i
1.95 -0.4871795 i
2 -0.5 i
2.05 -0.5121951 i
2.1 -0.5238095 i
2.15 -0.5348837 i
2.2 -0.5454545 i
2.25 -0.5555556 i
2.3 -0.5652174 i
2.35 -0.5744681 i
2.4 -0.5833333 i
2.45 -0.5918367 i
2.5 -0.6 i
2.55 -0.6078431 i
2.6 -0.6153846 i
2.65 -0.6226415 i
2.7 -0.6296296 i
2.75 -0.6363636 i
2.8 -0.6428571 i
2.85 -0.6491228 i
2.9 -0.6551724
2.95 -0.6610169 i
3 -0.6666667 i
3.05 -0.6721311 i
3.1 -0.6774194 i
3.15 -0.6825397 i
3.2 -0.6875 i
3.25 -0.6923077 i
3.3 -0.6969697 i
3.35 -0.7014925 i
3.4 -0.7058824 i
3.45 -0.7101449 i
3.5 -0.7142857 i
3.55 -0.7183099 i
3.6 -0.7222222 i
3.65 -0.7260274 i
3.7 -0.7297297 i
3.75 -0.7333333 i
3.8 -0.7368421 i
3.85 -0.7402597 i
3.9 -0.7435897 i
3.95 -0.7468354 i
4 -0.75 i

